Lifelong Learning Starting From Zero

We present a deep neural-network model for lifelong learning inspired by several forms of neuroplasticity. The neural network develops continuously in response to signals from the environment. In the beginning, the network is a blank slate with no nodes at all. It develops according to four rules: (i) expansion, which adds new nodes to memorize new input combinations; (ii) generalization, which adds new nodes that generalize from existing ones; (iii) forgetting, which removes nodes that are of relatively little use; and (iv) backpropagation, which fine-tunes the network parameters. We analyze the model from the perspective of accuracy, energy efficiency, and versatility and compare it to other network models, finding better performance in several cases.

==> AGI 2019 Lifelong learning/fcn_definitions.tex <==
\usepackage{amsopn}
\DeclareMathOperator{\sustainability}{sustainability}
\DeclareMathOperator{\ActionAnd}{\blacktriangle}
\DeclareMathOperator{\Comb}{Comb}
\DeclareMathOperator{\Seq}{Seq}
\DeclareMathOperator{\Tran}{Tran}
\DeclareMathOperator{\Cond}{Cond}
\DeclareMathOperator{\random}{random}
\DeclareMathOperator{\explore}{explore}
\DeclareMathOperator{\exploit}{exploit}
\DeclareMathOperator{\utility}{utility}
